Determining the dominant partial wave contributions from angular distributions of single- and double-polarization observables in pseudoscalar meson photoproduction

This work presents a simple method to determine the significant partial wave contributions to experimentally determined observables in pseudoscalar meson photoproduction. First, fits to angular distributions are presented and the maximum orbital angular momentum $\text{L}_{\mathrm{max}}$ needed to achieve a good fit is determined. Then, recent polarization measurements for $\gamma p \rightarrow \pi^{0} p$ from ELSA, GRAAL, JLab and MAMI are investigated according to the proposed method. This method allows us to project high-spin partial wave contributions to any observable as long as the measurement has the necessary statistical accuracy. We show, that high precision and large angular coverage in the polarization data are needed in order to be sensitive to high-spin resonance-states and thereby also for the finding of small resonance contributions. This task can be achieved via interference of these resonances with the well-known states. For the channel $\gamma p \rightarrow \pi^{0} p$, those are the $N(1680)\frac{5}{2}^{+}$ and $\Delta(1950)\frac{7}{2}^{+}$, contributing to the $F$-waves.

==> expl3-generic.tex <==
%%
%% This is file `expl3-generic.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% expl3.dtx  (with options: `generic,loader')
%% 
%% EXPERIMENTAL CODE
%% 
%% Do not distribute this file without also distributing the
%% source files specified above.
%% 
%% Do not distribute a modified version of this file.
%% 
%% File: expl3.dtx Copyright (C) 1990-2015 The LaTeX3 Project
%%
%% It may be distributed and/or modified under the conditions of the
%% LaTeX Project Public License (LPPL), either version 1.3c of this
%% license or (at your option) any later version.  The latest version
%% of this license is in the file
%%
%%    http://www.latex-project.org/lppl.txt
%%
%% This file is part of the "l3kernel bundle" (The Work in LPPL)
%% and all files in that bundle must be distributed together.
%%
%% The released version of this bundle is available from CTAN.
%%
%% -----------------------------------------------------------------------
%%
%% The development version of the bundle can be found at
%%
%%    http://www.latex-project.org/svnroot/experimental/trunk/
%%
%% for those people who are interested.
%%
%%%%%%%%%%%
%% NOTE: %%
%%%%%%%%%%%
%%
%%   Snapshots taken from the repository represent work in progress and may
%%   not work or may contain conflicting material!  We therefore ask
%%   people _not_ to put them into distributions, archives, etc. without
%%   prior consultation with the LaTeX3 Project.
%%
%% -----------------------------------------------------------------------
\def\ExplFileName{expl3}
\def\ExplFileDescription{L3 programming layer}
\def\ExplFileDate{2015/07/30}
\def\ExplFileVersion{5724}
\let\ExplLoaderFileVersion\ExplFileVersion
\begingroup
  \def\tempa{LaTeX2e}
  \def\next{}
  \ifx\fmtname\tempa
    \def\next
      {%
        \PackageInfo{expl3}{Switching from generic to LaTeX2e loader}
        \RequirePackage{expl3} \relax \endinput
      }
  \fi
\expandafter\endgroup
\next
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname ver@\ExplFileName -generic.tex\endcsname\relax
\else
  \immediate\write-1
    {%
      Package \ExplFileName\space Info: The package is already loaded.
    }%
  \expandafter\endinput
\fi
\immediate\write-1
  {%
    Package: \ExplFileName\space
    \ExplFileDate\space v\ExplFileVersion\space
    \ExplFileDescription\space (loader)
  }
\expandafter\edef\csname ver@\ExplFileName -generic.tex\endcsname
  {\ExplFileDate\space v\ExplFileVersion\space \ExplFileDescription}
\expandafter\edef\csname l@expl@tidy@tl\endcsname
  {%
    \catcode64=\the\catcode64\relax
    \let\expandafter\noexpand\csname l@expl@tidy@tl\endcsname
      \noexpand\undefined
  }
\catcode64=11 %
\chardef \l@expl@check@declarations@bool = 0 %
\chardef \l@expl@log@functions@bool = 0 %
\let\expl@AtBeginDocument\AtBeginDocument
\def\AtBeginDocument#1{}
\expandafter\def\expandafter\l@expl@tidy@tl\expandafter
  {%
    \l@expl@tidy@tl
    \let\AtBeginDocument\expl@AtBeginDocument
    \let\expl@AtBeginDocument\undefined
  }
\input expl3-code.tex %
\cs_set_eq:NN \__iow_wrap_set:Nx \tl_set:Nx
\protected\def\GetIdInfoLog{}
\cs_set_protected:Npn \ProvidesExplFile
  {
    \group_begin:
      \char_set_catcode_space:n { `\  }
      \ProvidesExplFileAux
  }
\cs_set_protected:Npn \ProvidesExplFileAux #1#2#3#4
  {
    \group_end:
    \iow_log:x { File:~#1~#2~v#3~#4 }
  }
\tex_input:D
  l3
  \xetex_if_engine:TF
    { xdvipdfmx }
    {
      \bool_if:nTF
        {
             \cs_if_exist_p:N  \pdftex_pdfoutput:D
          && \int_compare_p:nNn \pdftex_pdfoutput:D > \c_zero
        }
        { pdfmode }
        { dvips }
    }
  .def \scan_stop:
\tex_input:D l3unicode-data.def \scan_stop:
\cs_undefine:N \ProvidesExplFile
\cs_undefine:N \ProvidesExplFileAux
\ExplSyntaxOff
\l@expl@tidy@tl
%% 
%%
%% End of file `expl3-generic.tex'.

